Breaking the Visual Shortcuts in Multimodal Knowledge-Based Visual Question Answering

Existing Multimodal Knowledge-Based Visual Question Answering (MKB-VQA) benchmarks suffer from "visual shortcuts", as the query image typically matches the primary subject entity of the target document. We demonstrate that models can exploit these shortcuts, achieving comparable results using visual cues alone. To address this, we introduce Relational Entity Text-Image kNowledge Augmented (RETINA) benchmark, automatically constructed using an LLM-driven pipeline, consisting of 120k training and 2k human-curated test set. RETINA contains queries referencing secondary subjects (i.e. related entities) and pairs them with images of these related entities, removing the visual shortcut. When evaluated on RETINA existing models show significantly degraded performance, confirming their reliance on the shortcut. Furthermore, we propose Multi-Image MultImodal Retriever (MIMIR), which enriches document embeddings by augmenting images of multiple related entities, effectively handling RETINA, unlike prior work that uses only a single image per document. Our experiments validate the limitations of existing benchmarks and demonstrate the effectiveness of RETINA and MIMIR. Our project is available at: Project Page.

==> RETINA_camera_ready/fig/curation_ui.tex <==
\begin{figure*}[t]
  \centering
    \includegraphics[width=0.8\linewidth]{img/curation_ui.pdf}
  \caption{
  \textbf{Human Curation User Interface} 
  An image, document title, a question, and an answer are presented for curation, along with guidelines for identifying common issues.
  }
  \label{fig:ui}
\end{figure*}


==> RETINA_camera_ready/fig/distractor_recall.tex <==
\begin{figure}[t]
    \centering
        \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{img/distractor_seen.pdf}
        \caption{Seen}
        \label{fig:distractor-seen}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{img/distractor_unseen.pdf}
        \caption{Unseen}

        \label{fig:distractor-unseen}
    \end{subfigure}
    \caption{
    \textbf{Robustness to Visual-similar Distractors.} {\modelname} (\textbf{\textcolor{figgreen}{green}}) and MuKA (\textbf{\textcolor{figbrightred}{red}}) curves show recall for distractor (dotted) and GT (solid) documents. Distractors are non-GT documents whose main entity matches the query image’s entity. 
    }
    \label{fig:distractor_recall}
\end{figure}



==> RETINA_camera_ready/fig/filtered_example.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{img/filtered_example.pdf}
    \caption{\textbf{Example of a Valid Question Filtered Out due to Evaluation Constraints.} While both the question and its answer are factually valid, multiple duck species may be as closely related to the mandarin duck (green) as the wood duck (red) is. This ambiguity complicates strict automated evaluation, which is why such samples are filtered from the test set.}
    \label{fig:bad_example}
    \vspace{-1em}
\end{figure}


==> RETINA_camera_ready/fig/method.tex <==
\begin{figure*}[t]
    \centering  
    \includegraphics[width=1.0\linewidth]{img/method.pdf}
    \caption{
    \textbf{Overview of {\modelname} Document Encoder Architecture.}
     (a) given a document, related named entities are identified with an LLM~\cite{bai2023qwen}, and corresponding images are collected from the KB; (b) textual, global image, and patch-level features are extracted, with patch features attending to textual features through cross-attention to yield multimodal features; and (c) entity token embeddings are incorporated into the textual features prior to cross-attention for richer contextualization; (d) the final document embedding jointly integrates textual, global, and multimodal features projected into the same embedding space.
    }
    \label{fig:main}
\end{figure*}


==> RETINA_camera_ready/fig/pipeline.tex <==
\begin{figure*}[t]
    \centering    
    \includegraphics[width=\linewidth]{img/pipeline.pdf}
    \caption{
    \textbf{{\datasetname} Generation Pipeline.} (a) constructs one-hop neighborhood graphs by extracting named entities (\textbf{\textcolor{gray}{gray}} box) related to the answer entity (white box) and their relations using an LLM (relations are omitted); (b) samples a query entity (\textcolor{figbrightred}{\textbf{red}}) and qualifying entity (\textcolor{figteal}{\textbf{teal}}) to form a target subgraph with the answer entity (\textcolor{figgreen}{\textbf{green}}); and (c) feeds the target subgraph into an LLM to generate a textual query and collect a corresponding image from M2KR Images~\cite{lin2024preflmr}. The query is then paraphrased to minimize lexical overlap with the document.}
    \label{fig:pipeline}
\end{figure*}

==> RETINA_camera_ready/fig/prompt_entity_extraction.tex <==
\begin{figure*}[t]
\begin{tcolorbox}[colframe=gray!50!black, colback=gray!10!white, title=Entity extraction prompt, width=\textwidth, sharp corners=southwest]
\scriptsize
\begin{verbatim}
You are a Named Entity Recognition and Relation Extraction system specialized for 
identifying entities that
correspond to Wikipedia article title.

Your task is to extract all distinct named entities mentioned or referenced in the 
passage that align with
Wikipedia article titles, even if they are not exact substrings.

Guidelines:
1. For each entity, return an object with the fields: "entity", "entity_type", 
and "relation".
2. The "entity" must be a canonical Wikipedia title or a close variant that accurately 
represents the mention 
in the passage.
3. "entity_type" describes the category of the entity (e.g., Person, Place, 
Organization, Event, Book, Law, etc.).
You may create new types as needed.
4. The "relation" must follow these strict rules:
   - It must be a single, full natural language sentence.
   - The sentence must explicitly include the main entity as the subject.
   - It must describe concrete and fact-based relationships to the given entity, 
   including specific information 
   such as dates, functions, locations, roles, historical context, or other verifiable 
   details.
   - If there are multiple distinct factual relations for the entity, combine them 
   into one coherent 
   and grammatically correct sentence.
   - The sentence must be informative enough to support downstream question generation 
   tasks.
   - Avoid abstract, vague, or generic relations (e.g., "is related to", "is part of", 
   or incomplete phrases).
5. If the passage does not provide any clear relation for the entity, set "relation" 
to null.
6. Merge variations or aliases of the same entity to avoid duplication.
7. Be comprehensive and tolerant of indirect mentions or paraphrased references.

Wikipedia Title: "{entity}"

Passage:
\end{verbatim}
\end{tcolorbox}
\caption{\textbf{Entity Extraction Prompt.}}
\label{fig:entity_extraction_prompt}
\end{figure*}

==> RETINA_camera_ready/fig/prompt_paraphrasing.tex <==
\begin{figure*}[t]
\begin{tcolorbox}[colframe=gray!50!black, colback=gray!10!white, title=Paraphrasing Prompt, width=\textwidth, sharp corners=southwest]
\scriptsize
\begin{verbatim}
You are a helpful assistant that rewrites trivia questions only.  
Keep the original meaning and difficulty but change the wording.  
Do NOT include the answer in your response — output ONLY the rewritten question.  

Rewrite the following location-based trivia question using different wording,  
but keep the original meaning and difficulty level.  

Output format:  
Question: [your rewritten question]  
\end{verbatim}
\end{tcolorbox}
\caption{\textbf{Paraphrasing Prompt.}}
\label{fig:paraphrase}
\end{figure*}

==> RETINA_camera_ready/fig/prompt_question_generation.tex <==
\begin{figure*}[t]
\begin{tcolorbox}[colframe=gray!50!black, colback=gray!10!white, title=Question Generation Prompt, width=\textwidth, sharp corners=southwest]
\scriptsize
\begin{verbatim}
You are a VQA question-answer pair generator.

Given:
- Answer entity (answer to the question)
- Query entity (depicted in the image)
- Query entity's relation sentence describing how main and related entities 
are connected
- Qualifying entity's relation sentence describing the main entity

Generate a single, grammatically correct question-answer pair satisfying:

- The question refers indirectly to the query entity shown in the image by including 
exactly one singular 
demonstrative phrase matching the query entity’s type, e.g. "this country", 
"this building", "this city", etc.
- Do NOT explicitly name the query entity in the question.
- The demonstrative phrase must appear exactly once and without any article 
(no "a", "an", or "the").
- The question must use only the query entity's relation and/or qualifying entity's 
relation to describe the answer entity indirectly.
- The answer must be exactly the answer entity’s name.
- Do NOT mention or describe the image explicitly 
(no "shown here", "in this image", etc.).
- Output the question and answer in the format:

Question: [your question]  
Answer: [main entity]
\end{verbatim}
\end{tcolorbox}
\caption{\textbf{Question Generation Prompt.}}
\label{fig:qa_gen}
\end{figure*}

==> RETINA_camera_ready/fig/prompt_vila_retriever.tex <==
\begin{figure}[t]
\centering
\begin{tcolorbox}[colframe=gray!50!black, colback=gray!10!white,
  title=VILA Training Prompt, width=\columnwidth, sharp corners=southwest,
  boxsep=2pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
\scriptsize
\begin{alltt}
<image>
Question: {question}

Retrieved passages:
1: <image>{document_text_1}
2: <image>{document_text_2}
3: <image>{document_text_3}
4: <image>{document_text_4}
5: <image>{document_text_5}

Given the query image and question,
identify matched passages and provide a short answer.
\end{alltt}
\end{tcolorbox}
\caption{\textbf{VILA Training Prompt.}}
\label{fig:vila_prompt}
\vspace{-0.5em}
\end{figure}

\begin{figure}[t]
\centering
\begin{tcolorbox}[colframe=gray!50!black, colback=gray!10!white,
  title=Retriever Instruction Prompts, width=\columnwidth, sharp corners=southwest,
  boxsep=2pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
\scriptsize
\begin{alltt}
 <Image> Using the provided image, obtain
documents that address the subsequent question:

<Image> Retrieve documents that provide an
answer to the question alongside the image: 

<Image> Extract documents linked to the
question provided in conjunction with the image:

<Image> Utilizing the given image, obtain
documents that respond to the following question:

<Image> Using the given image, access documents that 
provide insights into the following question: 

<Image> Obtain documents that correspond to
the inquiry alongside the provided image: 

<Image> With the provided image, gather documents 
that offer a solution to the question: 

<Image> Utilizing the given image, obtain
documents that respond to the following question:
\end{alltt}
\end{tcolorbox}
\caption{\textbf{Retriever Instruction Prompts.}}
\label{fig:preflmr_prompt}
\vspace{-1.5em}
\end{figure}

==> RETINA_camera_ready/fig/qualitative_retina.tex <==
\begin{figure*}[t]
  \centering
    \includegraphics[width=\linewidth]{img/qualitative_retina.pdf}
  \caption{\textbf{Qualitative Examples of {\datasetname} Training Set before Human Curation.}}
  \label{fig:qualitative_qa}
\end{figure*}


==> RETINA_camera_ready/fig/qualitative_retrieval.tex <==
\begin{figure*}[t]
  \centering
    \includegraphics[width=\linewidth]{img/qualitative_retrieval.pdf}
  \caption{
  \textbf{Qualitative Comparison of Retrieval on {\datasetname} Benchmark.} Results for (a) MuKA~\cite{deng-etal-2025-muka} and (b) {\modelname}. GT documents are in \textbf{\textcolor{figgreen}{green}}; hard distractors containing the query image entity are in \textbf{\textcolor{figbrightred}{red}}; query entity in GT documents are highlighted in \textbf{\textcolor{figgreen}{green}}. 
  While MuKA is biased toward visual shortcuts and often retrieves documents containing images similar to the query, {\modelname} leverages related images 
  \protect\raisebox{-0.4ex}{\includegraphics[height=2ex]{img/qualitative_icon_1.pdf}} (Fraxinus americana) and \protect\raisebox{-0.4ex}{\includegraphics[height=2ex]{img/qualitative_icon_2.pdf}} (Nunavut), which are augmented to the document embeddings.%
  }
  \label{fig:examples}
\end{figure*}


==> RETINA_camera_ready/fig/shortcut_preliminary.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{img/shortcut_infoseek.pdf}
        \caption{Infoseek}
        \label{fig:shortcut-infoseek}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{img/shortcut_evqa.pdf}
        \caption{EVQA}

        \label{fig:shortcut-evqa}
    \end{subfigure}

    \caption{
        \textbf{Preliminary Experiment on Existing Benchmarks.}
        Recall@$k$ on benchmarks such as Infoseek~\cite{chen2023can} and EVQA~\cite{mensink2023encyclopedic},
        which exhibit visual shortcuts~\cite{deng-etal-2025-muka}.
        Models fine-tuned with image-only (\textbf{\textcolor{blue}{blue}}) queries versus image+text (\textbf{\textcolor{figgreen}{green}}) queries.
    }
    \label{fig:shortcut}
\end{figure}



==> RETINA_camera_ready/fig/shortcut_retina.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{img/shortcut_retina.pdf}
    \caption{\textbf{Image-only vs. Multimodal retrieval.} On EVQA (left), image-only MuKA (\textcolor{blue}{blue}) nearly matches the multimodal model (\textcolor{green!60!black}{green}), revealing the visual shortcut. On {\datasetname} (right), {\modelname} shows a substantial gap, indicating that multimodal processing is required.}
    \label{fig:shortcut_clarification}
\end{figure}


==> RETINA_camera_ready/fig/teaser.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{img/teaser.pdf}
    \caption{
    \textbf{Comparison of Previous MKB-VQA Benchmarks and {\datasetname}.} 
    (a) In previous benchmarks, the query image corresponds to the same visual entity (\textcolor{figbrightred}{\textbf{red}}) as (c) the shared GT document, creating a visual shortcut. (b) In {\datasetname}, the query uses a different visual entity (\textcolor{figgreen}{\textbf{green}}), breaking the visual shortcut.
    }
    \label{fig:task}
\end{figure}

==> RETINA_camera_ready/sec/01_intro.tex <==
\section{Introduction}
\label{sec:intro}
Knowledge-Based Visual Question Answering (KB-VQA) requires reasoning beyond the image and its natural language query, drawing on external knowledge to answer correctly. 
Central to this task is a multimodal retriever that identifies the target document from the visual and textual query.

\input{fig/teaser}
However, existing MKB-VQA benchmarks~\cite{10.1145/3477495.3531753, chen2023can, mensink2023encyclopedic, shahMYP19} share a construction choice that induces a \textit{visual shortcut}: the query image depicts the same entity as the target document's main entity, so the target is largely retrievable through visual similarity alone, without utilizing the textual evidence.
As shown in \Cref{fig:task}a and \cref{fig:task}c, the query and document images depict the exact same entity—the building ``Michigan Central Station''—enabling trivial retrieval.
Our preliminary experiment confirms this shortcut exploitation: we trained a baseline retriever~\cite{deng-etal-2025-muka} without the textual query to isolate its reliance on visual cues.
As shown in \Cref{fig:shortcut}, the retriever achieves comparable performance using the query image alone. 
Moreover, in practice, relevant information often resides in related documents rather than those directly depicting the query image.
For instance, in \Cref{fig:task}b, given a photo of \textit{Detroit} and the question “Which cycling path traverses the dam of this city and extends through Cumbria county?'', the answer resides not in the “Detroit'' document but in the ``Michigan Central Station'' document—rendering visual cues alone insufficient for retrieval.

\input{tab/benchmark_comparison}

To address this challenge, we construct {\datasetfullname} ({\datasetname}), an MKB-VQA benchmark with 120K training and 2K human-verified test samples, designed to eliminate visual shortcuts and better reflect real-world scenarios.
Prior benchmarks address a well-posed task in which the answer lies in the document of the depicted entity. 
{\datasetname} does not supersede them; it targets the complementary case, where the answer lies in a related document.
{\datasetname} serves as a counterbalance to existing shortcut-biased benchmarks.
Given the difficulty of manual construction, we build {\datasetname} via an automated LLM-driven pipeline. 
We introduce graph-based annotation as an intermediate step, leveraging graph structures to guide the LLM through relation extraction and query recomposition~\cite{ainslie2023gqa, tran2025reasonvqa, trivedi2022musiquemultihopquestionssinglehop, reddy-etal-2017-generating}. In particular, this allows us to decouple the complex generation process into structured sub-tasks, circumventing the reliance on direct prompting—a regime where LLMs are known to falter under compositional constraints~\cite{wen2024benchmarking} and suffer from degradation over long context windows~\cite{liu2023lostmiddlelanguagemodels}.
This strategy enables controlled generation by conditioning on target subgraphs of specific entities.

The same inductive bias is present on the model side, though it enters through the setup rather than the architectures.
Each document carries a single main-entity image, so that is what any retriever~\cite{deng-etal-2025-muka, lin2023finegrainedlateinteractionmultimodalretrieval, long2025retrieval, wei2024uniir, yu2025cafeunifyingrepresentationgeneration, lin2024preflmr} has to encode.
We confirm this inductive bias experimentally.
On {\datasetname}, existing retrievers tend to rank documents whose main-entity image matches the query above the related document that contains the answer.
We propose {\modelfullname} ({\modelname}), a retrieval framework that relaxes this inductive bias by representing each document with images of multiple related entities rather than a single main-entity image.
Specifically, {\modelname} extracts related entities from each document and collects their images, which are fused into the document embedding to guide retrieval when the query depicts one of these entities.
% [Original] This multi-image augmentation enables retrieval even without visual shortcuts.
\added{What matters is not the number of indexed images but their relation to the document: with the index size held fixed, neither additional views of the main entity nor images of unrelated entities recover the gain, which arises only when the indexed images depict the document's related entities (\cref{sec:capacity}).}
Experiments show that {\modelname} nearly doubles recall on {\datasetname} while matching or improving on existing MKB-VQA benchmarks.
Our contributions are as follows:
\begin{itemize}[itemsep=2pt, topsep=3pt, parsep=0pt, leftmargin=*]
\item We identify that visual shortcuts let retrievers recover the target from the query image alone in existing MKB-VQA benchmarks;
\item We propose an automatic graph-based pipeline that constructs shortcut-free samples;
\item We introduce {\datasetname}, a human-curated benchmark that counterbalances prior ones, enabling holistic evaluation with and without shortcuts;
\item 
% [Original] We propose {\modelname}, a retrieval framework that addresses the 
% [Original] visual shortcut.
\added{We propose {\modelname}, a retriever that identifies each document's related entities and indexes their images, and show that its gains stem from this entity association rather than from added index capacity.}
\end{itemize}
\added{The benchmark and the method form a single argument: {\datasetname} reveals the failure, and {\modelname} confirms its cause with a minimal fix, showing that knowledge about related entities must be made visually matchable at the document level.}



==> RETINA_camera_ready/sec/02_related_work.tex <==
\input{fig/shortcut_preliminary}
\section{Related Works}
\label{sec:related_works}
\input{fig/pipeline}
\noindent \textbf{Knowledge-Based VQA Benchmarks} 
Knowledge-based VQA datasets can be categorized by the modality of their external knowledge bases. Benchmarks relying solely on textual knowledge include SK-VQA~\cite{su2024sk}, S3VQA and OKVQAS3~\cite{jain2021select}, OK-VQA~\cite{marino2019okvqavisualquestionanswering}, A-OKVQA~\cite{schwenk2022aokvqabenchmarkvisualquestion}, and FVQA~\cite{wang2017fvqa}, requiring models to retrieve and reason over textual documents. A second group employs multimodal knowledge bases pairing documents with images, including KVQA~\cite{shahMYP19}, ViQuAE~\cite{10.1145/3477495.3531753}, Infoseek~\cite{chen2023can}, and E-VQA~\cite{mensink2023encyclopedic}; M-BEIR~\cite{wei2024uniir} also features a multimodal knowledge base but targets instructed retrieval rather than KB-VQA. Finally, some datasets integrate diverse modalities: M2KR~\cite{lin2024preflmr} spans both textual and multimodal resources, while WebQA~\cite{chang2022webqa} requires retrieval over heterogeneous sources of images or text, often with multi-hop queries.
\Cref{tab:benchmark_comparison}, compares {\datasetname} with existing MKB-VQA benchmarks.
Prior benchmarks~\cite{shahMYP19, 10.1145/3477495.3531753, chen2023can, mensink2023encyclopedic} pair each question with an image of the target document's \emph{main entity}, introducing the visual shortcut.
As shown in \cref{tab:benchmark_comparison} {\datasetname} is the only benchmark whose query images depict \emph{related} entities, requiring retrievers to jointly reason over visual and textual signals.

\noindent \textbf{Multimodal Retrievers} 
Foundational multimodal retrievers such as CLIP~\cite{radford2021learning}, Image-to-Word~\cite{Mori1999ImagetowordTB}, and BiT~\cite{kolesnikov2020bigtransferbitgeneral} align visual and textual representations in a shared embedding space for cross-modal retrieval. To handle queries combining text and images, this paradigm has been extended by ReVIVE~\cite{lin2022revive}, FLMR~\cite{lin2023finegrainedlateinteractionmultimodalretrieval}, and MuKA~\cite{deng-etal-2025-muka}, among other joint-modality architectures~\cite{Gao_2022_CVPR, long2025retrieval}. Universal frameworks—UniIR~\cite{wei2024uniir}, CAFE~\cite{yu2025cafeunifyingrepresentationgeneration}, MMEmbed~\cite{lin2025mmembeduniversalmultimodalretrieval}, GENIUS~\cite{kim2025genius}, LAMRA~\cite{liu2025lamra}, and PreFLMR~\cite{lin2024preflmr}—further support arbitrary query and document modalities. Despite these advances, existing retrievers encode each document with a single image, limiting retrieval on {\datasetname}, where queries involve diverse related entities. {\modelname} addresses this via multi-image encoding, yielding robust representations.

\added{\noindent \textbf{Multimodal Knowledge Graph RAG} \ 
Another line of work structures the knowledge base itself as a multimodal knowledge graph. RAG-Anything~\cite{guo2025raganything} builds cross-modal graphs over documents with hybrid graph and vector retrieval, and mKG-RAG~\cite{yuan2025mkgrag} constructs modality-aligned entity graphs for knowledge-intensive VQA with a dual-stage document-then-graph retrieval. These are full RAG pipelines that retrieve graph nodes and subgraphs for a generator, whereas {\modelname} is a document retriever that keeps the KB unchanged and only enriches each document's representation with images of its related entities, without typed relations or graph reasoning. We compare against both under a shared protocol in \cref{app:kgrag}.}


==> RETINA_camera_ready/sec/03_dataset.tex <==
\section{Dataset Construction}
\label{sec:pipeline}
We introduce {\datasetname}, a benchmark addressing the visual shortcut bias in existing MKB-VQA benchmarks. Unlike prior benchmarkss, queries in {\datasetname} cannot be solved through visual shortcuts, providing a balanced assessment when combined with prior benchmarks. For scalability, we develop an automated LLM-driven generation pipeline (\Cref{fig:pipeline}), yielding 120K training set and a 2K human-curated test set.

\subsection{MKB-VQA Sample Generation Pipeline}
While LLMs exhibit strong reasoning capabilities, their instruction-following degrades over long contexts such as Wikipedia~\cite{liu2023lostmiddlelanguagemodels}. We overcome this with a graph-based approach that ensures controllable generation, essential for maintaining the intended benchmark structure. Specifically, our pipeline comprises three stages: (a) converting the document into a knowledge graph, (b) selecting target subgraphs, and (c) generating multimodal QA from selected subgraphs.

\noindent{\textbf{Knowledge Graph Construction}} \ \
Wikipedia documents center on a primary subject, which we call the main entity. They typically contain an image of this entity, but using it as the query image introduces a visual shortcut. To circumvent this, we construct a one-hop graph centered on the main entity to identify related entities within the document, then generate queries paired with images of these related entities instead—keeping the benchmark shortcut-free.
To extract these entities, we prompt an LLM to identify named entities that co-occur with the main entity and bear a semantic relationship to it. Importantly, we do not fully convert the document into a structured entity–relation graph, as this often discards contextual information in the natural language—causal descriptions, attributes, temporal dependencies, and explanatory qualifiers. Instead, each edge is annotated with a natural language sentence describing the entity's relationship to the main entity. This representation enables precise control over target-entity selection for QA generation while preserving the original descriptive detail. \Cref{fig:pipeline}a illustrates this process: for the Wikipedia page on `Pennine Cycleway', the LLM identifies related entities such as `Scammonden Reservoir' and `Cumbria county' as neighboring nodes in the one-hop graph.

\noindent{\textbf{Target Subgraph Extraction}} \ \ 
MKB-VQA samples involve two related concepts: one depicted by the query image and one serving as the answer. 
Grounding QA in the Wikipedia KB, we instantiate these concepts as two entities per document: the main entity and a randomly selected related entity.
Since using the main entity as the query image would reintroduce the visual shortcut, we assign it as the answer entity and the related entity as the query entity.
Each pair, together with the tagged sentence describing their relation, forms the basis of an MKB-VQA sample.
However, questions formulated directly from this pair can be ambiguous, with multiple entities validly satisfying the question.
For example, in \Cref{fig:pipeline}b, the relation `The Pennine Cycleway crosses a dam at Scammonden Reservoir' with a query image of the reservoir may yield `Which cycling path traverses the dam of this reservoir?'---which admits multiple correct answers.
Since fully removing such ambiguity is difficult in an automated pipeline, we reduce it by introducing a qualifying entity: an additional randomly selected related entity that provides contextual cues to narrow down the answer.
The final target subgraph---query, answer, and qualifying entities---is passed to the LLM to generate the QA.

\noindent{\textbf{LLM-based VQA Sample Generation}} \ \ 
Given a target subgraph, we generate a QA sample comprising a query image, query text, and answer text.
We first retrieve an image of the query entity from M2KR~\cite{lin2024preflmr} as the query image.
We then prompt the LLM to formulate a question answered by the answer entity, conditioned on the two relation descriptions in the subgraph.
To ensure the query image is indispensable, the LLM is instructed to refer to the query entity not by name but with a demonstrative phrase (\eg, ``this organization'' or ``this monument'').
Finally, the question is paraphrased by the LLM, and we discard questions whose source document is retrieved by BM25~\cite{robertson1995okapi} in the top-5 results, reducing lexical overlap.
Full prompts are in the Appendix; \Cref{fig:pipeline}c illustrates the process with an example QA pair.

\subsection{{\datasetname} Bench Construction}
Following this procedure, we construct {\datasetname} using Qwen-2.5-32B-Instruct~\cite{bai2023qwen}, comprising a 120K training set and a 2K test set.
For the test set, we additionally apply a strict human selection stage that retains queries with an unambiguous answer that require both modalities to solve---a stricter bar than prior MKB-VQA benchmarks apply, ensuring automatic evaluation is reliable (\eg, a question such as ``What is the name of the plant that can be found in this state as well as in Florida?'' admits multiple valid answers and is excluded for evaluation; see \cref{app:curation}).
\added{We distinguish \emph{factual validity} from \emph{evaluation strictness}: a human audit finds 98.4\% of generated samples factually valid, but only 29.16\% also satisfy answer uniqueness and multimodal necessity. Rejected samples are mostly correct questions with multiple valid answers (75.35\%) or ones solvable without the image (21.27\%); they remain valid retrieval supervision and are kept for training (\cref{app:curation,app:train_quality}).
Accordingly, the shortcut-free property holds for both splits by construction, since every query image depicts a related rather than the main entity, while the test set is additionally verified by humans to require both modalities.}
We divide the test set into a seen subset, whose GT documents overlap with the training data, and an unseen subset without such overlap.
Finally, to guarantee a single GT document per query, we remove related entities whose documents reciprocally reference the main entity, preventing cases where both documents would reveal the answer.



==> RETINA_camera_ready/sec/04_method.tex <==
\input{fig/method}
\section{Method}
\label{sec:method}
Existing multimodal retrievers~\cite{deng-etal-2025-muka,caffagni2025recurrence,wei2024uniir} typically encode each document with a single image depicting its main entity.
While effective on existing MKB-VQA benchmarks, they falter on {\datasetname}: since document embeddings carry only the main entity's image, retrieval often fails when the query image depicts a non-main entity of the target document.
To address this, we introduce {\modelname}, a multimodal retriever whose core mechanism enriches document representations with images of multiple related entities, plus two lightweight, near-parameter-free refinements detailed below.
{\modelname} builds upon MuKA~\cite{deng-etal-2025-muka}, a single-image document retriever, extending its representation capacity.
Below, we review MuKA's scoring mechanism and query encoder (\cref{sec:late_interaction,sec:query_emb}), then detail our extended document embedding module (\cref{sec:doc_emb}).

\subsection{Late Interaction Scoring}
\label{sec:late_interaction}
Following the ColBERT family of multimodal retrievers~\cite{deng-etal-2025-muka, lin2024preflmr}, we represent the query and document as sets of token vectors, $\mathcal{Q} = \{ q_1, \dots, q_m \}$ and $\mathcal{D} = \{ d_1, \dots, d_n \}$.
Each query token contributes its maximum similarity over all document tokens, and these contributions are summed to yield the relevance score:
\begin{equation}
s(\mathcal{Q}, \mathcal{D}) = \sum_{i=1}^{m} \max_{j \in [1, n]} \text{sim}(q_i, d_j),
\end{equation}
where $\text{sim}(\cdot,\cdot)$ denotes cosine similarity.
Despite the token-wise computation, efficient indexing~\cite{santhanam2022plaidefficientenginelate} keeps retrieval practical.
This token-level formulation lets visual and textual query tokens match independently—visual tokens against similar document images, textual tokens against relevant text.

\subsection{Query Encoder}
\label{sec:query_emb}
The query encoder comprises image and text encoders and a cross-attention transformer block, each paired with dedicated projection layers.
Given a query $(I^{(q)}, T^{(q)})$, the goal is to produce the query feature set $\mathcal{Q}$ for scoring.
A ColBERTv2 text encoder~\cite{santhanam2022colbertv2effectiveefficientretrieval} yields $N_t$ token-level text embeddings $\mathcal{T}^{(q)} = \{t^{(q)}_{1}, \dots, t^{(q)}_{N_t}\}$, while a CLIP image encoder~\cite{radford2021learning} yields a global image feature $g^{(q)}$ and, from its penultimate layer, $N_p$ patch-level features $\mathcal{P}^{(q)} = \{p^{(q)}_{1}, \dots, p^{(q)}_{N_p}\}$.
The patch features are contextualized with the text via cross-attention~\cite{vaswani2023attentionneed}, using $\mathcal{P}^{(q)}$ as queries and $\mathcal{T}^{(q)}$ as keys and values, producing $N_p$ multimodal features $\mathcal{M}^{(q)} = \{m^{(q)}_{1}, \dots, m^{(q)}_{N_p}\}$.
Finally, $g^{(q)}$, $\mathcal{T}^{(q)}$, and $\mathcal{M}^{(q)}$ are projected into $\mathbb{R}^{D}$ by their dedicated projection layers (denoted $\widehat{\cdot}$), and concatenated to form the query feature set $\mathcal{Q} = [\widehat{g}^{(q)}; \widehat{\mathcal{T}}^{(q)}; \widehat{\mathcal{M}}^{(q)}]$.

\subsection{Document Encoder}
\label{sec:doc_emb}
\Cref{fig:main} overviews our document encoder.
Each document consists of a text and a main-entity image, following~\citet{deng-etal-2025-muka}.
We (a) augment it with images of related entities collected from the KB, (b) encode the text and all images into textual and visual features, (c) fuse each image with its relevant text via a multimodal mapping layer, where an Entity Token Embedding (ETE) marks the tokens of the entity depicted in each image, and (d) concatenate all features into the document representation $\mathcal{D}$.
We describe each step below.

\noindent{\textbf{(a) Augmenting Documents with Related Entity Images}} \ \
Given the textual content $T^{(d)}$, we identify all named entities related to the main entity with Qwen2.5-32B~\cite{bai2023qwen}, query the KB for each entity's document, and use its primary image as the entity's visual representation.
The augmented document is $(I^{(d)}_0, I^{(d)}_1, \dots, I^{(d)}_R, T^{(d)})$, where $I^{(d)}_0$ depicts the main entity and $I^{(d)}_r$, $r \in \{1,\dots,R\}$, depict related entities.
Note that we use an LLM only because the Wikipedia passages in M2KR~\cite{lin2024preflmr} are distributed without hyperlink label; entities are subsequently filtered to those with a corresponding KB document, so the resulting set approximates the Wikipedia's hyperlink structure. 
In deployment, hyperlinks can be used directly without an LLM.
\added{The source of the links (LLM extraction or hyperlinks) is interchangeable; what is essential is that each added image depicts an entity that the document actually relates to. Images of unrelated entities or additional views of the main entity, even at the same index size, do not yield the gain (\cref{sec:capacity}).}
\\
\noindent{\textbf{(b) Textual and Visual Feature Extraction}} \ \
Using the same ColBERTv2 and CLIP encoders as the query encoder, we extract token-level textual features $\mathcal{T}^{(d)} = \{t^{(d)}_{1}, \dots, t^{(d)}_{N_t}\}$ from $T^{(d)}$, and a global feature $g^{(d)}_r$ and patch-level features $\mathcal{P}^{(d)}_r = \{p^{(d)}_{r,1}, \dots, p^{(d)}_{r,N_p}\}$ from each image $I^{(d)}_r$, $r \in \{0,\dots,R\}$.
\input{tab/main_results}
\\
\noindent{\textbf{(c) Entity-Aware Multimodal Feature Extraction}} \ \
To capture information available through joint modeling of both modalities, each image's patches are fused with the text by a multimodal mapping layer---a cross-attention transformer block.
Since each image corresponds to a known named entity in $T^{(d)}$, we expose this association to the fusion rather than leaving alignment entirely to implicit attention: an Entity Token Embedding $\theta_{\text{ETE}}$, a learnable vector, is added to the entity's tokens, forming an image-specific textual set $\mathcal{T}^{(d)}_r$ via $t^{(d)}_{s} \leftarrow t^{(d)}_s + \theta_{\text{ETE}}$ for all $s \in \mathcal{S}_r$, where $\mathcal{S}_r$ denotes the token indices of the entity of $I^{(d)}_r$ (\textcolor{gray}{gray} tokens in \cref{fig:main}c).
The mapping layer then attends from $\mathcal{P}^{(d)}_r$ (query) to $\mathcal{T}^{(d)}_r$ (key and value), producing multimodal features $\mathcal{M}^{(d)}_r = \{m^{(d)}_{r,1}, \dots, m^{(d)}_{r,N_p}\}$ that are explicitly grounded in each image's entity.
\\
\noindent{\textbf{(d) Final Document embeddings}} \ \
All features are projected into $\mathbb{R}^D$ and concatenated:
\begin{equation}
    \mathcal{D} = \left[ \left( \widehat{g}^{(d)}_r, \widehat{\mathcal{M}}^{(d)}_r \right)_{r=0}^R; \widehat{\mathcal{T}}^{(d)} \right].
\end{equation}
Under late interaction (\cref{sec:late_interaction}), a query image depicting any related entity can now match its corresponding $\widehat{g}^{(d)}_r$ or $\widehat{\mathcal{M}}^{(d)}_r$, enabling retrieval without the visual shortcut.
\\
\noindent{\textbf{Relation to MuKA}} \ \
{\modelname} extends MuKA, which encodes only $(I^{(d)}_0, T^{(d)})$ and Concatenates patches with the full, unmarked text.
Our extension adds no learnable parameters beyond $\theta_{\text{ETE}}$, isolating the gains to the enriched representation. \added{We verify in \cref{sec:capacity} that these gains are not explained by the larger document representation alone.}



==> RETINA_camera_ready/sec/05_experiments.tex <==
\section{Experiments}
\label{sec:experiments}
\subsection{Experimental Setup}
\label{sec:experimental_setup}
\noindent\textbf{Datasets} \ \ 
We evaluate on {\datasetname} and two existing benchmarks, EVQA~\cite{mensink2023encyclopedic} and InfoSeek~\cite{chen2023can}.
Since {\datasetname} excludes visual shortcuts while EVQA and InfoSeek contain them, their combination enables comprehensive assessment of realistic MKB-VQA scenarios.
{\datasetname} contains 120K training samples and a 2K human-curated test set; EVQA provides 167K training and 3.7K test samples; InfoSeek consists of 676K training samples---of which we sample 100K following~\citet{lin2024preflmr}---and 4.7K test samples.
All three knowledge bases consist of textual Wikipedia documents (\cref{app:kb}), augmented with a main-entity image following~\citet{deng-etal-2025-muka} and further enriched with related-entity images as described in \cref{sec:doc_emb}.

\noindent\textbf{Metrics} \ \
We evaluate both retrieval and answer generation.
For retrieval, we report Recall@$K$, the proportion of queries whose annotated document appears in the top-$K$ results.
For generation, we use BERT Matching (BEM)~\cite{bulian-etal-2022-tomayto} on {\datasetname} and EVQA---a soft semantic measure beyond strict lexical matching---and InfoSeek's official Accuracy metric with answer-type-specific matching functions~\cite{chen2023can}.
Unless otherwise specified, all retrievers are evaluated by feeding their top-5 results to the same VILA-13B~\cite{liu2023visualinstructiontuning}, following~\citet{deng-etal-2025-muka}.

\noindent\textbf{Models} \ \
We compare {\modelname} against four multimodal baselines: UniIR~\cite{wei2024uniir}, ReT~\cite{caffagni2025recurrence}, PreFLMR~\cite{lin2024preflmr}, and MuKA~\cite{deng-etal-2025-muka}.
{\modelname}, PreFLMR, and MuKA share the same core encoders (ColBERT-base-v2 for text, CLIP ViT-G for vision) and differ mainly in the document encoder: PreFLMR uses text-only documents, MuKA attaches a single main-entity image, and {\modelname} incorporates multiple related-entity images (\cref{sec:doc_emb}).
Implementation details are in \cref{app:details}.

\subsection{Results}
\noindent\textbf{Evaluating Robustness Against Visual Shortcuts} \ \
We evaluate retrievers on {\datasetname}, InfoSeek, and EVQA, finetuning all models on the combined EVQA and {\datasetname} training sets to cover settings both with and without visual shortcuts.
As shown in \cref{tab:main}, single-image multimodal retrievers struggle on RETINA—even falling behind text-only baselines. 
This reversal highlights the effect of visual shortcuts: single-image models overfit to shortcut cues. 
Yet text-only recall itself remains low (23.6/11.1), confirming neither modality alone suffices on RETINA.
By augmenting documents with multiple related-entity images, {\modelname} achieves nearly twice the recall of the best baseline on {\datasetname} while remaining robust on existing benchmarks.
We additionally report performance with GT documents as an upper bound.

\input{tab/cross_dataset_transfer}

\noindent\textbf{Cross-Dataset Transfer} \ \
\Cref{tab:transfer} reports cross-dataset transfer evaluations across InfoSeek, EVQA, and {\datasetname}. 
Baselines trained on InfoSeek or EVQA fail to generalize when evaluated on the shortcut-free setting of {\datasetname}, dropping below 10\% R@5 on unseen splits. 
In contrast, {\modelname} demonstrates strong cross-dataset generalization; even when trained exclusively on InfoSeek or EVQA, it achieves 32.7\% and 34.0\% R@5 on {\datasetname} Unseen, respectively. 
Furthermore, when trained on {\datasetname}, {\modelname} retains competitive performance when transferred back to InfoSeek (46.3\% R@5) and EVQA (58.7\% R@5). 
While a moderate performance drop is observed compared to in-domain training, {\modelname} avoids catastrophic performance degradation, showing that {\datasetname} provides generalizable supervision without overfitting to shortcut cues.

\input{fig/shortcut_retina}

\noindent\textbf{The Visual Shortcut} \ \
Existing benchmarks pair the query image with the GT document's main entity, so a dense visual signal can dominate the sparse textual match (\cref{sec:late_interaction}) and recover the target on its own (\cref{sec:intro}). {\datasetname} breaks this coupling by letting the query depict any related entity, and \cref{fig:shortcut_clarification} shows the consequence: on EVQA (left), image-only MuKA (\textcolor{blue}{blue}) retains nearly 90\% (\textcolor{green!60!black}{green}) at top-k cutoffs (e.g., Recall@5 and @10). On {\datasetname} (right), however, the image-only performance drops by nearly half. 

\input{fig/qualitative_retrieval}

\added{\noindent\textbf{Robustness to Visual-similar Distractors}} \ \ \added{Against hard distractors---non-GT documents whose main entity matches the query image---MuKA retrieves distractors more often than GT documents at Recall@1, whereas {\modelname} consistently ranks GT documents higher, showing that it relies on text as well as visual similarity (\cref{app:distractor}).}

\added{\noindent\textbf{Disentangling Capacity from Entity Association}}\label{sec:capacity} \ \ \added{Since {\modelname} indexes more vectors per document than single-image baselines, we test whether its gain stems from added capacity or from \emph{which} evidence is indexed (\cref{tab:capacity}).
Each control enlarges the document representation to {\modelname}'s index size: (i) +repr.\ adds indexed vectors; (ii) +augmented images attaches as many crops/flips of the main-entity image as {\modelname} adds images; (iii) +related passages appends to PreFLMR the passages of the \emph{same} related entities, in text instead of images.
(i) and (ii) do not help on {\datasetname}, so capacity alone does not explain the gain.
(iii) gains little on {\datasetname} while sharply degrading InfoSeek and EVQA: {\datasetname} queries refer to the entity only through the image, and the appended text turns non-GT documents into distractors.
Conversely, with the number of images fixed, replacing related-entity images with unrelated ones monotonically lowers R@5 (43.2 $\rightarrow$ 36.8 at 0$\rightarrow$30\%; \cref{tab:selection_noise}b).
The gain thus comes from indexing the appearance of the document's related entities, not from a larger representation.}

\input{tab/capacity_control}

\added{\noindent\textbf{Efficiency and Index Size}} \ \ \added{Related-entity images increase indexed tokens by 2.3$\times$, a one-time offline cost, but search cost does not grow proportionally: PLAID~\cite{santhanam2022plaidefficientenginelate} prunes candidates via centroid interaction and fully scores only a small candidate set. Latency is dominated by query encoding ($\sim$2\,s) rather than retrieval ($\sim$0.002\,s), and the query encoder is identical to that of the single-image baseline (\cref{app:efficiency}). $K$, the number of related-entity images per document, controls index growth: even $K{=}1$ surpasses MuKA (24.7 vs.\ 20.8 R@5 on Seen; \cref{tab:selection_noise}a), so $K$ can be capped to trade index size for recall.}

\noindent\textbf{Qualitative Analysis} \ \
\Cref{fig:examples} compares MuKA and {\modelname} on {\datasetname}.
While MuKA also account for text, they tend to be heavily dominated by visual similarity, leading to exploit shortcut biases (\eg, trees or snowy landscapes in \cref{fig:examples}a) that push the GT document down despite its text relevance (\eg, \textit{medicinal} in \cref{fig:examples}b).
In contrast, {\modelname} identifies related entities during document encoding---\eg, Fraxinus americana' and Nunavut' in \cref{fig:examples}b---and integrates their visual features into the document representation.
This integration explicitly boosts the GT document's visual similarity score, which would otherwise remain low, overshadowing the textual similarity.
Consequently, {\modelname} achieves a higher rank for the GT document through balanced visual and textual alignment.

\input{tab/component_ablation}

\noindent{\textbf{{\modelname} Component Ablation}} \ \
\cref{tab:03_ablation_tab} ablates multiple images (MI), multimodal features (MMF), and entity token embeddings (ETE) from \cref{sec:doc_emb}.
The baseline corresponds to the original MuKA; thus +MI directly measures multi-image augmentation on the strongest single-image baseline.
% [Original] Adding multiple images (+MI)—here simply concatenating the projected global features of the additional images, as MuKA lacks multimodal document features—accounts for most of the RETINA gain (seen: 20.8 → 38.1), the essential ingredient for shortcut-free retrieval.
\added{Adding the images of the related entities identified in \cref{sec:doc_emb}(a) (+MI)---whose projected global features are concatenated to the document representation, as MuKA lacks multimodal document features---accounts for most of the {\datasetname} gain (seen: 20.8 $\rightarrow$ 38.1). As shown in \cref{sec:capacity}, this gain comes from the entity association of the added images, not from their number.}
Furthermore, +MMF and +ETE add ~2 points at nearly zero parameter cost, the former by enriching the document representation and the latter by aligning cross-attention with image-relevant text tokens.



==> RETINA_camera_ready/sec/06_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We propose {\datasetname}, a novel MKB-VQA benchmark that eliminates the visual shortcut present in prior datasets. We show that existing models exploit this shortcut, limiting their practical utility. 
{\datasetname} features a human-curated test set and large-scale training data generated via automatic graph-based pipeline. 
We further introduce {\modelname}, a framework designed for retrieval without over-relying on visual shortcuts. \added{Capacity-controlled analyses show that its gains come from indexing images of each document's related entities rather than from a larger representation.} Extending to other modalities remains a promising direction.

==> RETINA_camera_ready/sec/07_limitations.tex <==
\section*{Limitations}
First, {\modelname} requires a higher indexing cost than single-image retrievers, as encoding the images of related entities increases offline processing time and index size. While per-query latency is largely unaffected, this storage overhead may become a burden for very large knowledge bases.
Second, {\datasetname} relies on an LLM for entity extraction and question generation, which may introduce model-specific biases. Only the test set is human-verified, so the training set may still contain ambiguous questions.
Finally, both {\datasetname} and {\modelname} are built on English Wikipedia, and their generalization to other domains, languages, and knowledge bases remains untested.

==> RETINA_camera_ready/sec/08_acknowledgements.tex <==
\section*{Acknowledgements}
\added{This research was supported by MSIT (IITP: IITP-2026-RS-2024-00436857, RS-2024-00398115, IITP-2026-RS-2020-II201819, IITP-2026-RS-2025-02304828, RS-2026-25507282, RS-2026-25585074; NRF: RS-2025-23523979), MCST (KOCCA: RS-2026-25506607, RS-2024-00345025), MND (RS-2026-25551943) and MSS (RS-2026-25549378). This research was also supported by the ``Advanced GPU Utilization Support Program'' funded by the Government of the Republic of Korea (MSIT), and by a research grant from Google.}


==> RETINA_camera_ready/tab/benchmark_comparison.tex <==
\begin{table*}[t]
    \centering
    \caption{\textbf{Comparison with Existing MKB-VQA Benchmarks.} {\datasetname} is the only benchmark in which the query image depicts a related entity rather than the main entity of the target document, eliminating the visual shortcut.}
    \setlength{\tabcolsep}{5pt}
    \scalebox{0.72}{
        \begin{tabular}{lcccccc}
        \toprule
        \textbf{Benchmark} & \textbf{\#Train} & \textbf{\#Test} & \textbf{Answer Type} & \textbf{Query Entity} & \textbf{Shortcut-Free} & \textbf{Auto Construction} \\
        \midrule
        KVQA~\cite{shahMYP19}                 & 165.7K & 18.3K & Entity      & GT Document Image & \xmark & \xmark \\
        ViQuAE~\cite{10.1145/3477495.3531753} & 1.2K   & 1.2K  & Span        & GT Document Image & \xmark & \xmark \\
        OVEN~\cite{hu2023opendomainvisualentityrecognition}                & 6M     & 24.9K & Entity      & GT Document Image & \xmark & \cmark \\
        InfoSeek~\cite{chen2023can}           & 676K   & 4.7K  & Entity/Span & GT Document Image & \xmark & \cmark \\
        EVQA~\cite{mensink2023encyclopedic}  & 167K   & 3.7K  & Span/Free   & GT Document Image & \xmark & \cmark \\
        \midrule
        \textbf{{\datasetname} (Ours)}        & 120K   & 2K    & Entity & \textbf{Related Entity Image} & \cmark & \cmark \\
        \bottomrule
        \end{tabular}}
    \label{tab:benchmark_comparison}
\end{table*}


==> RETINA_camera_ready/tab/capacity_control.tex <==
\begin{table}[t]
    \centering
    \revcolor
    \setlength{\tabcolsep}{3.5pt}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{llcccc}
        \toprule
        & & \textbf{InfoSeek} & \textbf{EVQA} & \multicolumn{2}{c}{\textbf{{\datasetname}}} \\
        \cmidrule(lr){5-6}
        \textbf{Method} & \textbf{Size-matched aug.} & & & Seen & Unseen \\
        \midrule
        PreFLMR & -- & 40.7 & 63.9 & 23.6 & 11.1 \\
        PreFLMR & + repr. & 41.0 & 64.2 & 24.2 & 12.4 \\
        PreFLMR & + related passages & 27.3 & 43.1 & 27.2 & 14.7 \\
        \midrule
        MuKA & -- & 51.7 & 64.9 & 20.8 & 8.6 \\
        MuKA & + repr. & 52.0 & 64.8 & 21.2 & 8.9 \\
        MuKA & + augmented images & 52.9 & 65.3 & 17.2 & 6.3 \\
        \midrule
        \textbf{{\modelname}} & -- & \textbf{53.3} & \textbf{65.8} & \textbf{43.2} & \textbf{36.9} \\
        \bottomrule
        \end{tabular}
    }
    \caption{\added{\textbf{Capacity-Controlled Comparison} (R@5). Each control enlarges the per-document representation to {\modelname}'s index size without adding related-entity visual content.}}
    \label{tab:capacity}
\end{table}


==> RETINA_camera_ready/tab/component_ablation.tex <==
\begin{table}[t]
\centering
\caption{
\textbf{{\modelname} Component Ablation.} 
Cumulative impact of components on retrieval performance: baseline, +MI (Multiple Images), +MMF (Multimodal Features), and +ETE (Entity Token Embedding).
}
\label{tab:03_ablation_tab}
\scalebox{0.65}{%
\begin{tabular}{l c c c c}
\toprule
 & \textbf{InfoSeek} & \textbf{EVQA} & \multicolumn{2}{c}{\textbf{\datasetname}} \\
\cmidrule(lr){4-5}
\textbf{Method} &  &  & Seen & Unseen \\
\specialrule{1pt}{2pt}{2pt}
Baseline (MuKA \cite{deng-etal-2025-muka}) & 51.7 & 64.9 & 20.8 & 8.6 \\ 
\quad + MI & 51.5 & 65.1 & 38.1 & 33.3 \\
\quad + MMF & 51.6 & 65.3 & 41.1 & 34.5 \\
\quad + ETE (Full {\modelname}) & 53.3 & 65.8 & 43.2 & 36.9 \\ 
\bottomrule
\end{tabular}
}
\end{table}


==> RETINA_camera_ready/tab/cross_dataset_transfer.tex <==
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{4pt}
    \scalebox{0.8}{
        \begin{tabular}{llcccc}
        \toprule
        & & \textbf{InfoSeek} & \textbf{EVQA} & \multicolumn{2}{c}{\textbf{{\datasetname}}} \\
        \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-6}
        \textbf{Train} & \textbf{Method} & & & Seen & Unseen \\
        & & R@5 & R@5 & R@5 & R@5 \\
        \midrule
        \multirow{3}{*}{\textbf{InfoSeek}}
        & PreFLMR & 43.3 & 62.4 & 18.5 & 7.9 \\
        & MuKA    & \textbf{54.0} & 63.8 & 17.4 & 7.7 \\
        & \textbf{{\modelname}} & 53.9 & \textbf{64.3} & \textbf{35.2} & \textbf{32.7} \\
        \midrule
        \multirow{3}{*}{\textbf{EVQA}}
        & PreFLMR & 41.2 & 64.4 & 19.9 & 9.0 \\
        & MuKA    & 51.9 & 65.8 & 18.3 & 8.3 \\
        & \textbf{{\modelname}} & \textbf{53.5} & \textbf{66.0} & \textbf{39.9} & \textbf{34.0} \\
        \midrule
        \multirow{3}{*}{\textbf{{\datasetname}}}
        & PreFLMR & 31.8 & 53.6 & 24.6 & 13.0 \\
        & MuKA    & 42.1 & 56.5 & 22.2 & 10.1 \\
        & \textbf{{\modelname}} & \textbf{46.3} & \textbf{58.7} & \textbf{44.0} & \textbf{37.6} \\
        \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Cross-dataset Transfer.} Rows indicate the training source, columns the evaluation target.}
    \label{tab:transfer}
\end{table}


==> RETINA_camera_ready/tab/dataset_stats.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Summary of Dataset Statistics.}}
\label{tab:dataset_stats}
\scalebox{0.75}{ 
\begin{tabular}{lr}
\toprule
\textbf{} & \textbf{Value} \\ 
\midrule
Number of Main Entities & 19,408 \\
Number of Extracted Relations & 66,244 \\
\midrule
Avg. Train Question Length (tokens) & 26.4 \\
Avg. Train Answer Length (tokens) & 5.8 \\
Avg. Test Question Length (tokens) & 28.0 \\
Avg. Test Answer Length (tokens) & 5.5 \\
\bottomrule
\end{tabular}
}
\end{table}


==> RETINA_camera_ready/tab/kg_rag.tex <==
\begin{table}[t]
\centering
\revcolor
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
& \textbf{InfoSeek} & \textbf{EVQA} & \multicolumn{2}{c}{\textbf{{\datasetname}}} \\
\cmidrule(lr){4-5}
\textbf{Method} & & & Seen & Unseen \\
\midrule
RAG-Anything~\cite{guo2025raganything} & 34.0 & 27.7 & 21.3 & 19.2 \\
mKG-RAG~\cite{yuan2025mkgrag} & 45.7 & 35.8 & 25.8 & 22.8 \\
mKG-RAG + MuKA & 48.4 & 37.2 & 28.2 & 24.9 \\
mKG-RAG + {\modelname} & 47.9 & 38.6 & 32.6 & 29.3 \\
\midrule
\textbf{{\modelname}} & \textbf{53.3} & \textbf{65.8} & \textbf{43.2} & \textbf{36.9} \\
\bottomrule
\end{tabular}
}
\caption{\added{\textbf{Comparison with Multimodal KG-RAG Methods} (R@5) on the same KB under a shared top-5 retrieval protocol.}}
\label{tab:kgrag}
\end{table}


==> RETINA_camera_ready/tab/main_results.tex <==
\begin{table*}[t]
\centering
\caption{
\textbf{Evaluating Robustness Against Visual Shortcuts}. Retrieval and QA performance are reported. All models are jointly trained on EVQA and {\datasetname}. The GT Document row represents an upper bound using gold knowledge. 
{\modelname} consistently outperforms prior methods in both settings with and without visual shortcuts, showing the benefit of leveraging multi-image context over single-image or text-only approaches.
}
\scalebox{0.75}{
\begin{tabular}{llcccccccc}
\toprule
& & \multicolumn{2}{c}{\textbf{InfoSeek}} & \multicolumn{2}{c}{\textbf{EVQA}} & \multicolumn{4}{c}{\textbf{{\datasetname}}} \\
\cmidrule[.01pt](lr){3-4} \cmidrule[.01pt](lr){5-6} \cmidrule[.01pt](lr){7-10}
 & & & & & & \multicolumn{2}{c}{Seen} & \multicolumn{2}{c}{Unseen} \\
\cmidrule[.01pt](lr){7-8} \cmidrule[.01pt](lr){9-10}
\textbf{Method} & \textbf{Document Modality} & Recall@5 & Acc & Recall@5 & BEM & Recall@5 & BEM & Recall@5 & BEM \\
\specialrule{1pt}{2pt}{2pt}
PreFLMR~\cite{lin2024preflmr} & text & 40.7 & 33.5 & 63.9 & 57.0 & \textcolor{black}{23.6} & 19.9 & 11.1 & 13.6 \\
UniIR~\cite{wei2024uniir} & text + single-image & 34.5 & 26.4 & 22.0 & 25.7 & \textcolor{black}{13.8} & 14.6 & 4.7 & 11.2 \\
ReT~\cite{caffagni2025recurrence} & text + single-image & 50.1 & 40.4 & 46.3 & 43.7 & \textcolor{black}{15.1} & 15.2 & 6.8 & 11.4 \\
MuKA~\cite{deng-etal-2025-muka} & text + single-image & 51.7 & 41.0 & 64.9 & 60.7 & \textcolor{black}{20.8} & 18.7 & 8.6 & 12.2 \\
\textbf{{\modelname} (Ours)} & \textbf{text + multi-image} & \textbf{53.3} & \textbf{43.2} & \textbf{65.8} & \textbf{62.2} & \textbf{43.2} & \textbf{32.7} & \textbf{36.9} & \textbf{31.6} \\
\cmidrule(lr){1-10}
\textcolor{gray}{GT Document} & \textcolor{gray}{--} & \textcolor{gray}{--} & \textcolor{gray}{76.5} & \textcolor{gray}{--} & \textcolor{gray}{88.2} & \textcolor{gray}{--} & \textcolor{gray}{68.5} & \textcolor{gray}{--} & \textcolor{gray}{70.2} \\
\bottomrule
\end{tabular}
}
\label{tab:main}
\end{table*}

==> RETINA_camera_ready/tab/selection_noise.tex <==
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{5pt}
    \scalebox{0.85}{
        \begin{tabular}{lcccc}
        \toprule
        \multicolumn{5}{c}{\textbf{(a) Image selection strategy} (Recall@5)} \\
        \midrule
        \textbf{Strategy} & $K{=}1$ & $K{=}2$ & $K{=}3$ & $K{=}4$ \\
        \midrule
        Random   & 22.5 & 27.8 & 35.9 & 39.2 \\
        Frequent & 24.7 & 28.4 & 38.4 & 41.3 \\
        \midrule
        \multicolumn{5}{c}{\textbf{(b) Noise robustness} (Recall@5)} \\
        \midrule
        \textbf{Noise rate} & 0\% & 10\% & 20\% & 30\% \\
        \midrule
        {\modelname} & 43.2 & 42.8 & 40.9 & 36.8 \\
        \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Image Selection and Noise Robustness} on {\datasetname}. (a) Both selection strategies improve consistently with $K$, with frequency-based selection slightly ahead. (b) {\modelname} degrades gracefully under noisy related-entity images, remaining stable up to 20\%. \added{Noise replaces the given fraction of related-entity images with images of unrelated entities while keeping the number of images per document, the architecture, and training fixed, so it varies only the correctness of the entity association.}}
    \vspace{-1em}
    \label{tab:selection_noise}
\end{table}


==> RETINA_camera_ready/tab/std.tex <==
\begin{table*}[t]
\centering
\caption{
\textbf{Standard deviation analysis}. Average retrieval performance and standard deviations of {\modelname} are reported.
}
\scalebox{0.75}{
\begin{tabular}{llcccc}
\toprule
\textbf{Method} & \textbf{Document Modality} 
& \textbf{InfoSeek} 
& \textbf{EVQA} 
& \textbf{{\datasetname} (Seen)} 
& \textbf{{\datasetname} (Unseen)} \\
\specialrule{1pt}{2pt}{2pt}
PreFLMR~\cite{lin2024preflmr} & text & 40.7 & 63.9 & 23.6 & 11.1 \\
UniIR~\cite{wei2024uniir} & text + single-image & 34.5 & 22.0 & 13.8 & 4.7 \\
ReT~\cite{caffagni2025recurrence} & text + single-image & 50.1 & 46.3 & 15.1 & 6.8 \\
MuKA~\cite{deng-etal-2025-muka} & text + single-image & 51.7 & 64.9 & 20.8 & 8.6 \\
\textbf{{\modelname} (Ours)} & \textbf{text + multi-image} & \textbf{53.3} ($\pm 0.5$) & \textbf{65.8} ($\pm 0.4$)& \textbf{43.2} ($\pm 0.5$)& \textbf{36.9} ($\pm 0.6$)\\
\bottomrule
\end{tabular}
}
\label{tab:std}
\end{table*}


==> RETINA_camera_ready/tab/vlm_backbones.tex <==
\begin{table}[t]
\centering
\caption{
\textbf{{\modelname} with Diverse VLM Backbones.} QA performance (BEM~\cite{bulian-etal-2022-tomayto}) with and without retrieval.
}
\label{tab:vlm_comparison}
\scalebox{0.75}{%
\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{Retrieval} & \textbf{Seen} & \textbf{Unseen} \\
\midrule
\multirow{2}{*}{VILA-13B \cite{lin2024vilapretrainingvisuallanguage}} & \xmark & 11.2 & 10.1 \\
 & \cmark & 32.7 
 & 31.6 
 \\
\midrule
\multirow{2}{*}{InternVL3-8B \cite{zhu2025internvl3}} & \xmark & 18.7 & 17.6 \\
 & \cmark & 41.3 
 & 39.2 
 \\
\midrule
\multirow{2}{*}{Qwen3-VL-8B \cite{yang2025qwen3}} & \xmark & 20.3 & 19.4 \\
 & \cmark & 45.7 
 & 43.9 
 \\
\midrule
\multirow{2}{*}{GPT-4o \cite{hurst2024gpt}} & \xmark & 35.6 & 37.5 \\
 & \cmark & 55.8 
 & 57.2 
 \\
\bottomrule
\end{tabular}
}
\end{table}

